AnalogNAS: A Neural Network Design Framework for Accurate Inference with Analog In-Memory Computing

The advancement of Deep Learning (DL) is driven by efficient Deep Neural Network (DNN) design and new hardware accelerators. Current DNN design is primarily tailored for general-purpose use and deployment on commercially viable platforms. Inference at the edge requires low latency, compact and power-efficient models, and must be cost-effective. Digital processors based on typical von Neumann architectures are not conducive to edge AI given the large amounts of required data movement in and out of memory. Conversely, analog/mixed signal in-memory computing hardware accelerators can easily transcend the memory wall of von Neuman architectures when accelerating inference workloads. They offer increased area and power efficiency, which are paramount in edge resource-constrained environments. In this paper, we propose AnalogNAS, a framework for automated DNN design targeting deployment on analog In-Memory Computing (IMC) inference accelerators. We conduct extensive hardware simulations to demonstrate the performance of AnalogNAS on State-Of-The-Art (SOTA) models in terms of accuracy and deployment efficiency on various Tiny Machine Learning (TinyML) tasks. We also present experimental results that show AnalogNAS models achieving higher accuracy than SOTA models when implemented on a 64-core IMC chip based on Phase Change Memory (PCM). The AnalogNAS search code is released: https://github.com/IBM/analog-nas

==> sections/old_introduction.tex <==
Recent technological advancements have made \acp{DNN} ubiquitous for many challenging tasks, such as image classification, speech recognition, and machine translation. This success has been accompanied by rising demand for \ac{DNN} architecture engineering, which is becoming increasingly difficult to perform manually, as the underlying complexity of \ac{DNN} architectures continues to increase.


Manually-designed architectures are often tailored for specific hardware platforms. For instance, MobileNet~\cite{Howard2017} uses a depthwise separable convolution that enhances \ac{CPU} performance, but is inefficient for GPU parallelization~\cite{Lu2022}. 
\ac{NAS} methods seek to find optimal architectures by maximizing the expectation of performance of the sampled architectures using a validation set. However, conventional NAS approaches do not take the underlying hardware into account while searching for the best architectures. Increasing complexity and hardware dependence has given rise to an emerging category of \ac{NAS}, entitled \textit{\ac{HW-NAS}}~\cite{Benmeziane2021}, which is the primary focus of this paper. 


\ac{HW-NAS} consists of methods that automatically identify efficient \ac{DNN} architectures for a specific target hardware platform. In contrast to traditional \ac{NAS} that focuses on searching for the most accurate architectures, \ac{HW-NAS} searches for high-accuracy models while optimizing other metrics such as robustness to noise, latency, power-consumption, and area~\cite{Benmeziane2021}.
Many works~\cite{proxylessnas, fbnet, hwprnas, micronas, micronet} have succeeded in designing \ac{DNN} architectures for tiny and resource-constrained devices using \ac{HW-NAS}. \ac{DL} tasks in such devices are simplified to fit their constrained resource availability.


% To benchmark these devices, the MLPerf~\cite{} benchmark is commonly used.proposed four tiny machine learning tasks: Image Classification, Visual Wake Words, Keyword Spotting, and Anomaly detection. MicroNet~\cite{} uses \ac{HW-NAS} to find an efficient \ac{DNN} architecture for each of these tasks for micro-controllers. 
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/drift_new.pdf}
    \caption{The effect of \ac{PCM} device drift after one day on standard \ac{CNN} architectures and one architecture (\texttt{Resnet NAS T500}) obtained using \ac{HW-NAS}, evaluated using CIFAR-10.}
    \label{fig:motivation}
\end{figure}


Using specialized hardware, various hardware accelerators have been proposed to support the parallel execution of \ac{MVM} operations, which is the most dominant operation when performing \ac{DNN} inference.  \acp{GPGPU}~\cite{gpgpu}, \acp{FPGA}~\cite{fpga}, and \acp{ASIC}~\cite{asics} are among the widely used DNN hardware accelerators. To further improve computing performance and energy efficiency, the \ac{IMC} paradigm is proposed~\cite{imcgeneral}.  \ac{IMC} couples memory and computation, to mitigate the well known Von-Neuman bottleneck. Compute and storage elements in \ac{IMC} processes are typically built using a variety of memistive (memristive?) device types, including \ac{RRAM}~\cite{}, \ac{MRAM}~\cite{}, and \ac{PCM}~\cite{}. 
% \textcolor{red}{A \ac{PCM}-based accelerator is composed of PCM crossbars that perform the parallel MACs in \ac{DNN}. We assign the \ac{DNN} weights to the PCM cells in these crossbars.}
% In the PCM crossbar, the digital-analog converters (DAC) transform the digital input data (e.g., the feature maps in convolutional neural networks) to analog voltages. The analog MACs are executed in the crossbar. The output currents are the results of MACs, and the analog-digital converters (ADC) transform the currents into digital values.

% \color{red}
% Because the MAC is directly done by Ohm's and Kirchhoff's laws, analog computing in the crossbar is more efficient than digital computing in supporting \ac{DNN} parallel MACs. However, some requirements exist for deploying the \ac{DNN} on a given PCM-based accelerator. (1) \ac{DNN} weights should be quantized since the number of PCM cells' conductance levels is limited. (2) Since DAC and ADC are used in the PCM crossbar, and the conversions affect the prediction accuracy, they should be modelled in the \ac{DNN}. (3) \ac{DNN} architecture should be noise resistant because of the PCM inherent noise and drift over time. 

Fig.~\ref{fig:motivation} depicts the effect of \ac{PCM} device drift on standard architectures and one architecture obtained using \ac{HW-NAS} evaluated using CIFAR-10. 
As can be seen, despite having a relatively small number of network parameters, the \ac{NAS} (T500) network is extremely robust to \ac{PCM} device drift.


% Since the existing \ac{DNN}s cannot match these requirements, it is desirable to design hardware-friendly networks, which can be deployed on the given PCM-based accelerator and perform good prediction accuracy under noise and drift effects. 
Current \ac{HW-NAS} strategies cannot be ported to \ac{IMC} accelerators without modification for two reasons: (i) their search space contains operations and blocks that are not suitable for analog devices. Such operations include depthwise seperable convolutions~\cite{Howard2017} and efficientnet block~\cite{efficientnetv2}, and (ii) their search strategy does not include noise and drift injection which searches for robust and resilient \ac{DNN} architectures.

This situation motivates us to use a novel \ac{HW-NAS} strategy to design dedicated \ac{DNN} architectures for deployment on \ac{IMC} inference accelerators which use analog devices for compute and storage. In this paper, we propose \texttt{AnalogNAS}, a \ac{HW-NAS} framework for analog dedicated \ac{NAS}. AnalogNAS considers these requirements to build the search space for which each network can be deployed. An evolution algorithm is used to explore the search space, which simulates biological evolution, including specialized mutations and selection. To compare different networks, we design a surrogate model, able to predict the rank of the architectures, as well as the drift effect after a month of inference. 
To verify the effectiveness of AnalogNAS, we perform exhaustive hardware simulations, and deploy a subset of network architectures on a real \ac{PCM}-based \ac{IMC} inference accelerator.
% search over a 960M sized search space and achieve a more robust, more efficient architecture on Analog Devices. 

Our specific contributions can be summarized as follows:
\begin{itemize}
    \item We design a Resnet-like Search Space. The search space is inspired by the Resnet~\cite{resnet} architecture and contains the standard resnet-like architectures, including ResNext~\cite{resnext} and Wide-Resnet~\cite{wideresnet}. The architectures within the search can have varying widths and depths and different blocks, which helps us get insights into the types of robust architectures best deployed in analog devices.
    \item We build a surrogate model to rank the architecture during the search and predict the drift robustness. Architecture training is done using hardware-aware training with noise injection. 
    \item Using the surrogate model, we propose a global search strategy that uses evolution search to explore the search space and efficiently finds the right architecture under different constraints, such as the number of parameters and number of used tiles.
    \item We conduct comprehensive experiments to demonstrate that AnalogNAS can be efficiently utilized to carry out architecture search for various tiny applications, including image classification, visual wake words, and keyword spotting. By analyzing the search population, we validate the intuition that the search tends to have wide architectures. 
\end{itemize}
